AutoDroid-V2: Boosting SLM-based GUI Agents via Code Generation

Large language models (LLMs) have brought exciting new advances to mobile UI agents, a long-standing research field that aims to complete arbitrary natural language tasks through mobile UI interactions. However, existing UI agents usually demand powerful large language models that are difficult to be deployed locally on end-users' devices, raising huge concerns about user privacy and centralized serving cost. Inspired by the remarkable coding abilities of recent small language models (SLMs), we propose to convert the UI task automation problem to a code generation problem, which can be effectively solved by an on-device SLM and efficiently executed with an on-device code interpreter. Unlike normal coding tasks that can be extensively pre-trained with public datasets, generating UI automation code is challenging due to the diversity, complexity, and variability of target apps. Therefore, we adopt a document-centered approach that automatically builds fine-grained API documentation for each app and generates diverse task samples based on this documentation. By guiding the agent with the synthetic documents and task samples, it learns to generate precise and efficient scripts to complete unseen tasks. Based on detailed comparisons with state-of-the-art mobile UI agents, our approach effectively improves the mobile task automation with significantly higher success rates and lower latency/token consumption. Code is open-sourced at https://github.com/MobileLLM/AutoDroid-V2.

==> tex/related_work.tex <==
\section{Related Work}\label{sec:related_work}
\yuanchun{Can be removed to save space}

\textbf{UI Task Automation} is to build systems that can execute tasks automatically based on the UI. The most relevant works can be categorized as 1. Understanding the semantic meaning of a GUI \cite{vut}. These methods can help summarize the main functions of a GUI \cite{spotlight}, understand the purpose of each control \cite{li-etal-2020-widget, screen_recognition}, and address user questions related to the GUI \cite{screen2words, breadown_conversations}. It is important for enabling various interaction tasks such as UI automation and accessibility.
2. Mapping the instructions from users to UI elements \cite{seq2act, metagui, kite}. These methods are to select the GUI element that is the most relevant to an instruction from the user. Recently, some works are using LLMs to map the instructions to GUI elements \cite{talking_with_ui}.
3. Mobile UI task automation \cite{responsible_task_automation, AITW_dataset,wen2023droidbot-gpt}. These methods build an agent to complete tasks from users by performing actions on the GUI. 
\name, on the other hand, leverages the automatically generated UI transition memory to complete high-level tasks including multiple steps on a smartphone. The memory can help agents to understand richly informative UIs and the usage of apps, and augment the LLMs in reasoning and planning.

\subsection{LLMs for Code Synthesis}
Large Language Models (LLMs) have demonstrated significant capability in code synthesis due to extensive training on vast code datasets \cite{openai2023gpt4, nijkamp2022codegen, gunasekar2023textbooks}. 
They are widely used in various applications, such as API calling \cite{qin2024toolllm, hugginggpt, gorilla}, test script generation \cite{LLM4Test, ryan2024code}, and device manipulation \cite{xu2024penetrative, code_as_policy}. 
In these scenarios, LLMs receive human tasks and interact with tools like APIs, Python interpreters, and DNN models. 
Acting as the brain, LLMs synthesize code to create high-level plans, operating these tools until the task is complete. 

\wh{is code better than single-step, offer an example in other fields, otherwise we can prove it. }

Building on the success of LLM-based code generation, we aim to extend this approach to UI manipulation. 
Existing LLM-based methods for interacting with mobile UIs to complete tasks \cite{wen2023droidbot-gpt, responsible_task_automation, autodroid, mm-navigator} typically follow a step-wise manner. 
These methods take user tasks and the current UI state (described in structured data and/or images) as inputs, and produce the next UI action in Text/JSON format. 
Recent works have shown that LLM agents synthesizing executable Python code are advantageous over Text/JSON actions due to programming knowledge \cite{wang2024executable}. 
Therefore, we propose using LLMs to generate high-level code encompassing multi-step operations in UI states, which would mitigate delays from querying LLMs at each step. 
Additionally, script-based methods can enhance accuracy by reducing hallucinations about lengthy UI action sequences and enable more complex tasks through the synthesis of complex control logic.


% \textbf{LLMs for Code Generation}
% Although LLMs can execute various tasks such as question answering and text generation, they are still limited by the information they can store in their fixed set of weights and the maximum context length. Therefore, researchers are trying to augment LLMs with various tools, such as web browser \cite{webgpt, mind2web}, various APIs \cite{chamelon, gorilla}, and even other models \cite{hugginggpt, gpt4tools, visual_programming}. These works often rely on cleverly designed prompts to improve the reasoning ability of LLMs or fine-tune LLMs on domain-specific dataset. Besides, they often suppose there are public-available APIs to solve tasks. Our method, however, does not relay on human-designed APIs that are not usual in mobile apps.

% \textbf{Process Mining} is the process of using software tools to automatically analyze the functionality, performance, and usability of Android applications. 
% Typical techniques include static analysis \cite{arzt2014flowdroid} (which analyzes the static components of mobile apps such as the code, resource files, configurations) and dynamic analysis \cite{enck2014taintdroid,droidbot} (which is focused on the runtime behavior).
% In mobile task automation, the key to understand the functionalities of the apps. Prior work has explored to extract such functionality information based on the code \cite{wang2017purpose}, GUI \cite{li2016peruim}, network traffic \cite{jin2018traffic_purpose}, and metadata \cite{guo2018feature_redundancy}, but they are mostly too coarse-grained to facilitate task completion.
% Our method uses LLMs to process the raw traces collected by a dynamic app analyzer \cite{droidbot} to obtain fine-grained description of each GUI element.

